Offline tagging of radon-induced backgrounds in XENON1T and applicability to other liquid xenon detectors

This paper details the first application of a software tagging algorithm to reduce radon-induced backgrounds in liquid noble element time projection chambers, such as XENON1T and XENONnT. The convection velocity field in XENON1T was mapped out using $^{222}\text{Rn}$ and $^{218}\text{Po}$ events, and the root-mean-square convection speed was measured to be $0.30 \pm 0.01$ cm/s. Given this velocity field, $^{214}\text{Pb}$ background events can be tagged when they are followed by $^{214}\text{Bi}$ and $^{214}\text{Po}$ decays, or preceded by $^{218}\text{Po}$ decays. This was achieved by evolving a point cloud in the direction of a measured convection velocity field, and searching for $^{214}\text{Bi}$ and $^{214}\text{Po}$ decays or $^{218}\text{Po}$ decays within a volume defined by the point cloud. In XENON1T, this tagging system achieved a $^{214}\text{Pb}$ background reduction of $6.2^{+0.4}_{-0.9}\%$ with an exposure loss of $1.8\pm 0.2 \%$, despite the timescales of convection being smaller than the relevant decay times. We show that the performance can be improved in XENONnT, and that the performance of such a software-tagging approach can be expected to be further improved in a diffusion-limited scenario. Finally, a similar method might be useful to tag the cosmogenic $^{137}\text{Xe}$ background, which is relevant to the search for neutrinoless double-beta decay.

==> rn_decay_chain.tex <==
\tikzstyle{block} = [rectangle, draw, fill=white, 
    text width=3.2em, text centered, rounded corners, minimum height=2em]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{figure*}
    \centering
    \begin{tikzpicture}[scale=1, node distance = 5.2cm, auto]
        \node at (0,0) [block] (U238) {\isotope{U}{238}};
        \node [block, right of=U238] (Th234) {\isotope{Th}{234}};
        \node [block, right of=Th234] (Pa234m) {\isotope{Pa}{234m}};
        \node [block, right of=Pa234m] (U234) {\isotope{U}{234}};
        \node at (0,-3cm) [block] (Th230) {\isotope{Th}{230}};
        \node [block, right of=Th230] (Ra226) {\isotope{Ra}{226}};
        \node [block, right of=Ra226] (Rn222) {\isotope{Rn}{222}};
        \node [block, right of=Rn222] (Po218) {\isotope{Po}{218}};
        \node at (0,-6cm) [block] (Pb214) {\isotope{Pb}{214}};
        \node [block, right of=Pb214] (Bi214) {\isotope{Bi}{214}};
        \node [block, right of=Bi214] (Po214) {\isotope{Po}{214}};
        \node [block, right of=Po214] (Pb210) {\isotope{Pb}{210}};
        \node at (0,-9cm) [block] (Bi210) {\isotope{Bi}{210}};
        \node [block, right of=Bi210] (Po210) {\isotope{Po}{210}};
        \node [block, right of=Po210] (Pb206) {\isotope{Pb}{206}};

        \draw [arrow] (U238) -- node [align=center, anchor=center]{\(Q(\alpha) = 4269.7 \pm 2.9 \unit{keV}\)\\ \\ \((4.468 \pm 0.003)\times10^6 \unit{yr}\)} (Th234);
        \draw [arrow] (Th234) -- node [align=center, anchor=center]{\(Q(\beta^-) = 273 \pm 3 \unit{keV}\)\\ \\ \(24.10 \pm 0.03 \unit{d}\)} (Pa234m);
        \draw [arrow] (Pa234m) -- node [align=center, anchor=center]{\(Q(\beta^-) = 2195 \pm 4 \unit{keV}\)\\ \\ \(1.159 \pm 0.011 \unit{min}\)} (U234);
        \draw [arrow] (U234) -- (15.6cm, -1.5cm) -- node [align=center, anchor=center]{\(Q(\alpha) = 4859.8 \pm 0.9 \unit{keV}\)\\ \\ \((2.455 \pm 0.006)\times10^5 \unit{yr}\)} (0cm, -1.5cm) -- (Th230);
        \draw [arrow] (Th230) -- node [align=center, anchor=center]{\(Q(\alpha) = 4770.0 \pm 1.5 \unit{keV}\)\\ \\ \((7.538 \pm 0.030)\times10^4 \unit{yr}\)} (Ra226);
        \draw [arrow] (Ra226) -- node [align=center, anchor=center]{\(Q(\alpha) = 4870.62 \pm 0.25 \unit{keV}\)\\ \\ \(1600 \pm 7 \unit{yr}\)} (Rn222);
        \draw [arrow] (Rn222) -- node [align=center, anchor=center]{\(Q(\alpha) = 5590.4 \pm 0.3 \unit{keV}\)\\ \\ \(3.8222 \pm 0.0002 \unit{d}\)} (Po218);
        \draw [arrow] (Po218) -- (15.6cm, -4.5cm) -- node [align=center, anchor=center]{\(Q(\alpha) = 6114.75 \pm 0.09 \unit{keV}\)\\ \\ \(3.097 \pm 0.012 \unit{min}\)} (0cm, -4.5cm) -- (Pb214);
        \draw [arrow] (Pb214) -- node [align=center, anchor=center]{\(Q(\beta^-) = 1018 \pm 11 \unit{keV}\)\\ \\ \(27.06 \pm 0.07 \unit{min}\)} (Bi214);
        \draw [arrow] (Bi214) -- node [align=center, anchor=center]{\(Q(\beta^-) = 3269 \pm 11 \unit{keV}\)\\ \\ \(19.71 \pm 0.02 \unit{min}\)} (Po214);
        \draw [arrow] (Po214) -- node [align=center, anchor=center]{\(Q(\alpha) = 7833.46 \pm 0.06 \unit{keV}\)\\ \\ \(163.6 \pm 0.3 \unit{\mu s}\)} (Pb210);
        \draw [arrow] (Pb210) -- (15.6cm, -7.5cm) -- node [align=center, anchor=center]{\(Q(\alpha) = 63.5 \pm 5 \unit{keV}\)\\ \\ \(22.20 \pm 0.22 \unit{yr}\)} (0cm, -7.5cm) -- (Bi210);
        \draw [arrow] (Bi210) -- node [align=center, anchor=center]{\(Q(\beta^-) = 1162.2 \pm 0.8 \unit{keV}\)\\ \\ \(5.012 \pm 0.005 \unit{d}\)} (Po210);
        \draw [arrow] (Po210) -- node [align=center, anchor=center]{\(Q(\alpha) = 5407.45 \pm 0.07 \unit{keV}\)\\ \\ \(138.376 \pm 0.002 \unit{d}\)} (Pb206);
    \end{tikzpicture}
    \caption{Only branches with branching fraction above \(99.5 \%\) are shown. {\color{red} Start at Rn-222 instead}}
    \label{fig:rn222_decay_chain}
\end{figure*}

==> rn_decay_chain_smaller.tex <==
\tikzstyle{block} = [rectangle, draw, fill=white, 
    text width=3.2em, text centered, rounded corners, minimum height=2em]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{figure*}
    \centering
    \begin{tikzpicture}[scale=1, node distance = 5.2cm, auto]
        \node at (0,0) [block] (Rn222) {\isotope{Rn}{222}};
        \node [block, right of=Rn222, text=blue, draw=blue] (Po218) {\isotope{Po}{218}};
        \node [block, right of=Po218, text=Maroon, draw=Maroon] (Pb214) {\isotope{Pb}{214}};
        \node [block, right of=Pb214, text=blue, draw=blue] (Bi214) {\isotope{Bi}{214}};
        \node at (0,-3cm) [block, text=blue, draw=blue] (Po214) {\isotope{Po}{214}};
        \node [block, right of=Po214] (Pb210) {\isotope{Pb}{210}};
        \node [block, right of=Pb210] (Bi210) {\isotope{Bi}{210}};
        \node [block, right of=Bi210] (Po210) {\isotope{Po}{210}};
        \node at (0,-6cm) [block] (Pb206) {\isotope{Pb}{206}};
        \node [below = 0.00cm of Pb206] (Pb206_label) {stable};

        \draw [arrow] (Rn222) -- node [align=center, anchor=center]{\(Q(\alpha) = 5590.4 \pm 0.3 \unit{keV}\)\\ \\ \(3.8222 \pm 0.0002 \unit{d}\)} (Po218);
        \draw [arrow] (Po218) -- node [align=center, anchor=center]{\(Q(\alpha) = 6114.75 \pm 0.09 \unit{keV}\)\\ \\ \(3.097 \pm 0.012 \unit{min}\)} (Pb214);
        \draw [arrow] (Pb214) -- node [align=center, anchor=center]{\(Q(\beta^-) = 1018 \pm 11 \unit{keV}\)\\ \\ \(27.06 \pm 0.07 \unit{min}\)} (Bi214);
        \draw [arrow] (Bi214) -- (15.6cm, -1.5cm) -- node [align=center, anchor=center]{\(Q(\beta^-) = 3269 \pm 11 \unit{keV}\)\\ \\ \(19.71 \pm 0.02 \unit{min}\)} (0cm, -1.5cm) -- (Po214);
        \draw [arrow] (Po214) -- node [align=center, anchor=center]{\(Q(\alpha) = 7833.46 \pm 0.06 \unit{keV}\)\\ \\ \(163.6 \pm 0.3 \unit{\mu s}\)} (Pb210);
        \draw [arrow] (Pb210) -- node [align=center, anchor=center]{\(Q(\beta) = 63.5 \pm 5 \unit{keV}\)\\ \\ \(22.20 \pm 0.22 \unit{yr}\)} (Bi210);
        \draw [arrow] (Bi210) -- node [align=center, anchor=center]{\(Q(\beta^-) = 1162.2 \pm 0.8 \unit{keV}\)\\ \\ \(5.012 \pm 0.005 \unit{d}\)} (Po210);
        \draw [arrow] (Po210)-- (15.6cm, -4.5cm) -- node [align=center, anchor=center]{\(Q(\alpha) = 5407.45 \pm 0.07 \unit{keV}\)\\ \\ \(138.376 \pm 0.002 \unit{d}\)} (0cm, -4.5cm) -- (Pb206);
    \end{tikzpicture}
    \caption{Decay chain of \isotope{Rn}{222}, part of the uranium series. Only branches with branching fraction above \(99.5 \%\) are shown. Data retrieved using the NNDC ENSDF, with relevant Nuclear Data Sheets citations \cite{Singh:2019qyr}, \cite{Zhu:2021qss}, \cite{ShamsuzzohaBasunia:2014yyr}, \cite{Kondev:2008roc}. The isotope that decays to produce the background events being tagged in this work, \isotope{Pb}{214}, is coloured maroon, whereas the isotopes with decays that are used for the tagging of \isotope{Pb}{214} are coloured blue.}
    \label{fig:rn222_decay_chain}
\end{figure*}
